Subsampling Methods for Persistent Homology

Persistent homology is a multiscale method for analyzing the shape of sets and functions from point cloud data arising from an unknown distribution supported on those sets. When the size of the sample is large, direct computation of the persistent homology is prohibitive due to the combinatorial nature of the existing algorithms. We propose to compute the persistent homology of several subsamples of the data and then combine the resulting estimates. We study the risk of two estimators and we prove that the subsampling approach carries stable topological information while achieving a great reduction in computational complexity.

==> framework__Brittany_Terese_Fasy_s_conflicted_copy_2014-06-06_.tex <==
%----------------------------------------------------------
\section{Background}
%----------------------------------------------------------
\label{sec:background}

Computing persistent homology requires building
a nested sequence of geometric complexes indexed by a real parameter.
In this section, we briefly introduce these families and topological summaries
of them, but refer the reader
to Section 4.2. of~\cite{cso-psgc-12} for a complete definition of these
geometric filtered complexes and their use in TDA, to
\cite{edelsbrunner2010computational} for the definition of persistence
diagrams, and to \cite{bubenik2012statistical} for the definition and properties
of
persistence landscapes.

% \subsection{Measured Metric Spaces}
%
% Let $( \X,\rho)$ denote a metric space, $\mathcal K(\X)$ the set of
% all the compact subsets of $\X$, and $H(C_1,C_2)$ the Hausdorff distance
% between two subsets $C_1, C_2 \in \mathcal K(\X)$; see
% \cite{burago2001course}.
% Two compact metric spaces $( \X_1,\rho_1)$ and $( \X_2,\rho_2)$ are {\em
% isometric} if there exists a bijection $\Phi : \X_1 \to \X_2$ that
% preserves distances, namely: $\forall x,y \in \X_1$, $\rho_2(\Phi(x),\Phi(y))
% = \rho_1(x,y)$. Such a map $\Phi$ is called an {\em isometry}.
% One way to
% compare two metric spaces is to measure how far these two metric spaces are
% from
% being isometric. The corresponding distance is called the {\em
% Gromov-Hausdorff
% distance} (see for instance \cite{burago2001course}). Intuitively, it is the
% infimum of their Hausdorff distance over all possible isometric embeddings of
% these two spaces into a common metric space.
% The Gromov-Hausdorff distance $\dgh$ defines a metric on
% the space $\mathcal K$
% of isometry classes of compact metric spaces (see Theorem 7.3.30 in
% \cite{burago2001course}).
% Notice that when $\X_1$ and $\X_2$ are subspaces of a same metric space
% $(\X, \rho)$ then $\dgh(\X_1,\X_2) \leq H(\X_1,\X_2)$.
%
% %\paragraph{Measure.}
% Let $\mu$ be a probability measure on $(\X,\rho)$ equipped with its Borel
% algebra.  Let $\X_\mu$
% denote the support of the measure $\mu$, namely the smallest closed set with
% probability one. Throughout the remainder of this paper, we will assume that
% $\X_\mu$ is compact and thus $\X_\mu \in \mathcal K (\X)$. Also note that
% $(\X_\mu, \rho)  \in \mathcal{K}$.


\subsection{Geometric Complexes}
\begin{figure}[ht!b!]
\centering
\includegraphics[height=2cm]{figs/complex1}\ \
\includegraphics[height=2cm]{figs/complex4}\ \
\includegraphics[height=2cm]{figs/complex2}\ \
\includegraphics[height=2cm]{figs/complex3}
\caption{From left to right: the $\alpha$ sublevelset of the distance function
to a point
  set $\X$ in $\R^2$, the $\alpha$-complex, $\Cech_\alpha(\X)$, and
$\Rips_{2\alpha}(\X)$.
The last two complexes include a tetrahedron.}
\label{fig:complex}
\end{figure}

To compute the persistent homology from a set of data,
we need to construct a set of structures called simplicial complexes.
A simplicial complex $\K$
is a set of simplices (points, segments, triangles, etc) such that any face
from a simplex in $\K$ is also in $\K$ and the intersection of any two
simplices of $\K$ is a (possibly empty) face of these simplices.

Given a metric space $\X$, we define three simplicial complexes that
use the zero-skeleton $\{ x_i \}_{x_i \in \X}$; see
Figure~\ref{fig:complex} for illustrations.  The
\emph{Vietoris-Rips complex} $\Rips_{\alpha}(\X)$ is the set of
simplices~$[x_0,\ldots,x_k]$ such that $d_{\X}(x_i,x_j)\leq \alpha$ for all
$(i,j)$.
The \emph{\v Cech complex} $\Cech_\alpha(\X)$ is similarly defined as
the set of simplices $[x_0,\ldots,x_k]$ such that there exists a point $x \in
\X$ for which $d_{\X}(x,x_i)\leq \alpha$ for all $i$.
%\footnote{When $\X$ is
%embedded in $\R^d$, we can extend
%the definition of the \v Cech complex to allow for $x \in \R^d$ instead of $x
%\in \X$.}
Note that these two complexes are related by
$\Rips_\alpha(\X)\subseteq\Cech_\alpha(\X)\subseteq\Rips_{2\alpha}(\X)$.
% Note that these two families of complexes only depend on the pairwise
%distances between the points of $\X$.
 We also define the
\emph{$\alpha$-complex} as
the set of simplices $[x_0,\ldots,x_k]$ such that the smallest circle defined
by the set of vertices $\{x_0, \ldots, x_k  \}$ contains no point of $\X$ in
the interior of the circle.
%While the Rips and the {\v C}ech complexes can have
%simplicies of dimension equal to the cardinality of $\X$, the
%$\alpha$-complex
%is a subcomplex of the
%Delaunay triangulation and thus only contains simplices of dimension at
%most~$d$.

%The {\v C}ech and $\alpha$-complexes have the same homology as the union of
%the balls $\bigcup_{x \in \X}
%B(x,\alpha)$.  Moreover, this union of the balls is also the
%$\alpha$-sublevel set of the
%distance function to $\X$, $d(\cdot,\X)$, and, as a consequence,
%increasing $\alpha$ from zero to infinity is a convenient way to study the
%evolution of the topology of the sublevel sets of $d(\cdot,\X)$.  We are
%interested in this evolution, as we can
%interpret a sublevel set of $d(\cdot, \X)$ as an estimate of the support of the
%distribution from which the points in $\X$ were drawn.


Each family described above is non-decreasing with
$\alpha$: for any $\alpha\leq\beta$, there is an inclusion of
$\Rips_\alpha(\X)$ in $\Rips_\beta(\X)$, and similarly for the \v Cech
and Alpha complexes. These sequences of inclusions are called
\emph{filtrations}.
In the following, we let $\Filt(\X) := (\Filt_\alpha (\X))_{\alpha
\in \mathcal A}$  denote  a filtration corresponding to one of the
parameterized complexes defined above.
%There are several other families that we
%could also have considered, most
%notably witness complexes, which were defined in \cite{cso-psgc-12}. Extending
%our results to them is
%straightforward and yields very similar results, so we will restrict to the
%families defined above in the rest of the paper.




\subsection{Persistence Diagrams}
The topology of $\Filt_\alpha (\X)$ changes as $\alpha$
increases: new connected components (cycles and cavities) appear, existing
components become connected, etc.
Persistent homology tracks these changes.
%, identifies the number
%of components, cycles, and cavaties as \emph{features}, and
%associates an \emph{interval} or \emph{lifetime} to each~feature.
%Intuitively, the longer a feature persists, the more relevant it is.
%More specifically, the features in which we are intersted are the ranks of the
%homology groups of the complexes. The homology of a space $\mathbb{X}$ is a
%collection of abelian groups of different dimensions; the $p$-dimensional
%group encodes the $p$-dimensional ``holes" in $S$.
%Formally, the $p$th
%homology group $H_p(\mathbb{X})$ is the set of equivalence classes of loops
%enclosing the
%$p$th dimensional holes, and its rank $\beta_p$ is called the $p$th
%\textit{Betti number}.
%The $p$th Betti number $\beta_p$ measures the number of
%$p$-dimensional holes in $\mathbb{X}$, so that $\beta_0$ is the number of
%connected
%components of $\mathbb{X}$, $\beta_1$ is the number of loops, $\beta_2$ is the
%number
%of enclosed voids and so on.
Each homological feature of $\Filt (\X)$  has a birth time $b$ and a
death time $d$. The
\emph{persistence diagram}~$\dgm(\Filt (\X))$ is the multiset of
birth-death pairs $\{ (b_i,d_i)
\}_{i \in I}$.
For technical reasons, we include all points
of the diagonal $\Delta$ with infinite multiplicity, i.e., $(b,b) \in
\dgm(\Filt (\X))$ for all $b \geq 0$.
We note here that $\dgm(\Filt(\mathbb{Y}))$ is well-defined for any
compact metric space $\mathbb{Y}$; see \cite{chazal2012structure,cso-psgc-12}.

We will abuse terminology slightly,
and let the \emph{persistence diagram of $\X$}, denoted by $D_{\X}$, refer
to~$D(\Filt (\X))$, the persistence diagram of an appropriate
filtration. To avoid (minor) technical difficulties, we restrict our attention
to
diagrams $D$ such that $(b,d) \in [0,T] \times [0,T]$ for all $(b,d) \in D$,
for some fixed $T>0$. We denote by
$\mathcal{D}_T$ the space of all such (restricted) persistence~diagrams.



%There are several options for how to represent a
%persistence diagram: as a barcode, as a diagram, or as a rotated diagram.   In
%this exposition, we choose the latter; the feature that is born at $b$ and
%dies at $d$ is represented by the point
%$(\frac{b+d}{2},\frac{d-b}{2})$; see~\figref{fig:landscape}.  In words,
%the $x$-coordinate is the average parameter value over which the feature
%exists,
%and the $y$-coordinate is the half-life of the feature.

The space of persistence diagrams is endowed with a metric called the
\emph{bottleneck distance}, denoted by $\bottle$.
Let the distance between two pairs $(b_i,d_i)$ and $(b_j,d_j)$ be the maximum
between $|b_i-b_j|$ and $|d_i-d_j|$.
Given two persistence
diagrams, the bottleneck distance is
defined as the infimum value $\delta$ for which we can find a perfect matching
between
the diagrams such that two points can only be matched if their distance is less
than $\delta$.
The presence of the diagonal in all diagrams means we can consider partial
matchings of the off-diagonal points, and the remaining points are matched to
the~diagonal.

A fundamental property of persistence diagrams, proven in
\cite{chazal2012structure}, is their \emph{stability}.
Given a metric space $(\mathbb{X},\rho)$, the Hausdorff distance is
defined as
$\displaystyle
\dhaus(X,Y)= \max \Big\{ \max_{x \in X} \min_{y \in Y} \rho(x,y) , \;  \max_{y
\in Y}
\min_{x \in X} \rho(x,y) \Big\},
$
for any $X,Y \subset \mathbb{X}$.
If $\X$ and $\tilde \X$
are two compact metric spaces, then one has
\begin{equation} \label{bot-dgh}
\bottle\left(
\dgm (\Filt(\X)),
\dgm (\Filt(\tilde \X))
\right)
~\leq~
2 \dgh \left(\X, \tilde \X\right),
\end{equation}
where $\dgh  \left(A,B \right)$ denotes the Gromov-Hausdorff distance,
i.e., the
infimum Hausdorff distance between the two compact sets $A$ and $B$
over all possible isometric embeddings into a common metric space.
Moreover, if $\X$ and $\tilde \X$ are embedded in the same metric space
$(\X,\rho)$ then (\ref{bot-dgh}) holds for the Hausdorff distance~$\dhaus(\cdot,
\cdot)$ in place of $2\dgh(\cdot,\cdot)$.
% Note that these properties are intrinsic to the metrics defined on $\X$ and
% $\tilde \X$; they do not involve any probability
% measure.  Later in this paper, we will be interested in understanding the
% persistent homology of the support of a probability measure.



%\begin{figure}[ht!b!]
%\centering
%\includegraphics[height=1.5in]{figs/triangles3b}\ \
%\includegraphics[height=1.5in]{figs/triangles-CI}
%\caption{The pink circles represent the points in a persistence diagram $D$.
%          As shown on the left, the landscape $\lscape(k, \cdot)$ is the $k$-th
%          largest
%          of the arrangement of the graphs of $\{ \Lambda_p \}$.
%          In particular, the cyan curve is the landscape $\lscape(1,\cdot)$.
%          On the right, we see a confidence interval for this landscape.}
%\label{fig:landscape}
%\end{figure}

\subsection{Persistence Landscapes}

The persistence landscape, introduced in \cite{bubenik2012statistical},
is a collection of continuous, piecewise linear
functions~\mbox{$\lscape \colon  \Z^{+} \times \R \to \R$} that summarizes a
persistence diagram.
To define the landscape, consider the set of functions created by tenting
each each point $p=(x,y)= \left( \frac{b+d}{2}, \frac{d-b}{2}  \right)$
representing a birth-death pair $(b,d) \in D$ as follows:
\begin{equation}\label{eq:triangle}
 \Lambda_p(t) =
 \begin{cases}
  t-x+y & t \in [x-y, x] \\
  x+y-t & t \in (x,  x+y] \\
  0 & \text{otherwise}
 \end{cases}
 =
 \begin{cases}
  t-b & t \in [b, \frac{b+d}{2}] \\
  d-t & t \in (\frac{b+d}{2}, d] \\
  0 & \text{otherwise}.
 \end{cases}
\end{equation}
%Notice that $p$ is itself on the graph of $\Lambda_p(t)$.

\begin{wrapfigure}{L}{0.5\textwidth}
% \vspace{-10pt}
\centering
	\includegraphics[height=1.5in]{figs/triangles3b}\ \
\caption{
	We use the rotated axes to represent a persistence diagram $D$.
	A feature $(b,d) \in D$ is represented by the point
	$(\frac{b+d}{2},\frac{d-b}{2})$ (pink).
	In words,
	the $x$-coordinate is the average parameter value over which the feature
exists,
	and the $y$-coordinate is the half-life of the feature.
        The cyan curve is the landscape $\lscape(1,\cdot)$.}
\label{fig:landscape}
 \vspace{-15pt}
\end{wrapfigure}

We obtain
an arrangement of piecewise linear curves by overlaying the graphs of
the functions~\mbox{$\{ \Lambda_p \}_{p}$}; see~\figref{fig:landscape}.

The persistence landscape of $\dgm$ is a  summary of this arrangement.
Formally, the persistence landscape of $D$ is the collection of functions
\begin{equation}\label{eq:landscape}
 \lscape_{\dgm}(k,t) = \underset{p}{\text{kmax}} ~ \Lambda_p(t), \quad
 t \in [0,T], k \in \mathbb{N},
\end{equation}
where kmax is the $k$th largest value in the set; in particular,
$1$max is the usual maximum~function. We set $\lscape_{\dgm}(k,t) = 0$ if the
set $\{ \Lambda_p(t)\}_p$ contains less than
$k$ points.  For simplicity of exposition, if $D_{\X}$ is the persistence
diagram of some metric space $\X$, then we use
$\lambda_{\X}$ to denote $\lambda_{D_{\X}}$.

We denote by $\lscapespace$ the space
of persistence landscapes corresponding to
$\dgmspace$.
From the definition of persistence landscape, we immediately observe that
$\lscape_{\dgm}(k,\cdot)$ is one-Lipschitz.
%,  since the composite functions $\Lambda_p$ are one-Lipschitz.
%  Hence, for all $\lambda \in \lscapespace$, $\lambda$
%is one-Lipschitz and vanishes outside of $(0,T)$; therefore, the landscape
%$\lambda$ is upper bounded by $T/2$.
The following additional properties are proven in \cite{bubenik2012statistical}.

\begin{lemma} \label{lemma:basic-prop}
Let $D, D'$ be persistence diagrams. We have the following for any $t\in
\mathbb{R}$ and any $k \in \mathbb{N}$:\\
(i)  $\lambda_D(k,t)
~\geq~ \lambda_D(k+1,t) ~\geq~ 0 $.\\
(ii) $| \lambda_D(k,t) - \lambda_{D'}(k,t)| ~\leq~  \bottle(D,D')$.
\end{lemma}
For ease of exposition, we focus on the case $k=1$,
and set $\lscape_D(t) = \lscape_{\dgm}(1,t)$.  However,
the results we present hold for~$k > 1$.  In fact, the results hold for more
general summaries of persistence landscapes, including the silhouette defined
in \cite{chazal2013stochastic}. %\\ % for spacing with the wrapfigure


==> latex/Makefile <==
all: refman.pdf

pdf: refman.pdf

refman.pdf: clean refman.tex
	pdflatex refman
	makeindex refman.idx
	pdflatex refman
	latex_count=5 ; \
	while egrep -s 'Rerun (LaTeX|to get cross-references right)' refman.log && [ $$latex_count -gt 0 ] ;\
	    do \
	      echo "Rerunning latex...." ;\
	      pdflatex refman ;\
	      latex_count=`expr $$latex_count - 1` ;\
	    done


clean:
	rm -f *.ps *.dvi *.aux *.toc *.idx *.ind *.ilg *.log *.out *.brf *.blg *.bbl refman.pdf

